Examples of renormalized SDEs

We demonstrate two examples of stochastic processes whose lifts to geometric rough paths require a renormalisation procedure to obtain convergence in rough path topologies. Our first example involves a physical Brownian motion subject to a magnetic force which dominates over the friction forces in the small mass limit. Our second example involves a lead-lag process of discretised fractional Brownian motion with Hurst parameter $H \in (1/4,1/2)$, in which the stochastic area captures the quadratic variation of the process. In both examples, a renormalisation of the second iterated integral is needed to ensure convergence of the processes, and we comment on how this procedure mimics negative renormalisation arising in the study of singular SPDEs and regularity structures.

==> preamble.tex <==
\usepackage{amsfonts}
\usepackage{amsmath, amsthm}
\usepackage{color}
\usepackage{amsfonts}
\usepackage{amssymb}
%\usepackage{mathtools}
\usepackage{hyperref}

\usepackage{shuffle}
%\usepackage[all]{xy}
%\usepackage[utf8]{inputenc} 
%\usepackage{comment}

\RequirePackage[inline]{enumitem}
\RequirePackage[numbers]{natbib}

%\usepackage{hyperref}
%\usepackage{breakurl}

\usepackage{mathrsfs}
%\usepackage{enumitem}
%
\usepackage{tikz}
%\usepackage{dsfont}
\usepackage{mhequ} 
%\usepackage{mhsymb} 
%\usepackage{mhenvs} 
%\usepackage{array}
%
%\usepackage{wasysym}
%\usepackage{centernot}
%
%\setlist{noitemsep,nolistsep,leftmargin=1.7em}
%\parindent1em
% 
\usetikzlibrary{snakes}
\usetikzlibrary{decorations}
\usetikzlibrary{positioning}
\usetikzlibrary{shapes}
\usetikzlibrary{external}
\tikzexternalize[prefix=tikz/]

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
%
%              Some tikz code to draw nice trees
%
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


\makeatletter
\pgfdeclareshape{crosscircle}
{
  \inheritsavedanchors[from=circle] % this is nearly a circle
  \inheritanchorborder[from=circle]
  \inheritanchor[from=circle]{north}
  \inheritanchor[from=circle]{north west}
  \inheritanchor[from=circle]{north east}
  \inheritanchor[from=circle]{center}
  \inheritanchor[from=circle]{west}
  \inheritanchor[from=circle]{east}
  \inheritanchor[from=circle]{mid}
  \inheritanchor[from=circle]{mid west}
  \inheritanchor[from=circle]{mid east}
  \inheritanchor[from=circle]{base}
  \inheritanchor[from=circle]{base west}
  \inheritanchor[from=circle]{base east}
  \inheritanchor[from=circle]{south}
  \inheritanchor[from=circle]{south west}
  \inheritanchor[from=circle]{south east}
  \inheritbackgroundpath[from=circle]
  \foregroundpath{
    \centerpoint%
    \pgf@xc=\pgf@x%
    \pgf@yc=\pgf@y%
    \pgfutil@tempdima=\radius%
    \pgfmathsetlength{\pgf@xb}{\pgfkeysvalueof{/pgf/outer xsep}}%  
    \pgfmathsetlength{\pgf@yb}{\pgfkeysvalueof{/pgf/outer ysep}}%  
    \ifdim\pgf@xb<\pgf@yb%
      \advance\pgfutil@tempdima by-\pgf@yb%
    \else%
      \advance\pgfutil@tempdima by-\pgf@xb%
    \fi%
    \pgfpathmoveto{\pgfpointadd{\pgfqpoint{\pgf@xc}{\pgf@yc}}{\pgfqpoint{-0.707107\pgfutil@tempdima}{-0.707107\pgfutil@tempdima}}}
    \pgfpathlineto{\pgfpointadd{\pgfqpoint{\pgf@xc}{\pgf@yc}}{\pgfqpoint{0.707107\pgfutil@tempdima}{0.707107\pgfutil@tempdima}}}
    \pgfpathmoveto{\pgfpointadd{\pgfqpoint{\pgf@xc}{\pgf@yc}}{\pgfqpoint{-0.707107\pgfutil@tempdima}{0.707107\pgfutil@tempdima}}}
    \pgfpathlineto{\pgfpointadd{\pgfqpoint{\pgf@xc}{\pgf@yc}}{\pgfqpoint{0.707107\pgfutil@tempdima}{-0.707107\pgfutil@tempdima}}}
  }
}
\makeatother




\def\XiTwoTwo{\tikz[baseline=0.5,scale=0.15]{\draw (0,0) node[xi] {} -- (-1,1) node[not] {} -- (0,2) node[xi] {};}}

\def\XiTwoX{\tikz[baseline=-2,scale=0.15]{\draw (0,-0.25) node[xi] {} -- (-1,1) node[xix] {};}}

\def\XiThree{\tikz[baseline=0,scale=0.15]{\draw (0,0) node[xi] {} -- (-1,1) node[xi] {} -- (0,2) node[xi] {};}}
\def\IXiTwo{\tikz[baseline=0,scale=0.15]{\draw (0,-0.25) node[not] {} -- (-1,1) node[xi] {} -- (0,2) node[xi] {};}}
\def\XiThreeb{\tikz[baseline=-1,scale=0.15]{\draw (-1,1) node[xi] {} -- (0,0) node[xi] {} -- (1,1) node[xi] {};}}
\def\XiFourd{\tikz[baseline=-4.5,scale=0.15]{\draw (0,-1.5) node[not] {} -- (0,0); \draw (-1,1) node[xi] {} -- (0,0) node[xi] {} -- (1,1) node[xi] {};}}
\def\IXiIXi{\tikz[baseline=-1,scale=0.15]{\draw (-1,1) node[xi] {} -- (0,0) node[not] {} -- (1,1) node[xi] {};}}

\def\XiFour{\tikz[baseline=2,scale=0.15]{\draw (0,0) node[xi] {} -- (-1,1) node[xi] {} -- (0,2) node[xi] {} -- (-1,3) node[xi] {};}}
\def\IXiThree{\tikz[baseline=2,scale=0.15]{\draw (0,-0.25) node[not] {} -- (-1,1) node[xi] {} -- (0,2) node[xi] {} -- (-1,3) node[xi] {};}}
\def\XiOne{\tikz[baseline=-2.8,scale=0.15]{\node[xib] {};}}
\def\XiX{\tikz[baseline=-2.8,scale=0.15]{\node[xibx] {};}}
\def\IXi{\tikz[baseline=-2,scale=0.15]{\draw (0,-0.25) node[not] {} -- (-1,1) node[xi] {};}}
\def\XiI{\tikz[baseline=-2,scale=0.15]{\draw (0,-0.25) node[xi] {} -- (-1,1) node[not] {};}}
\def\IXiX{\tikz[baseline=-1,scale=0.15]{\draw (0,-0.25) node[not] {} -- (-1,1) node[xix] {};}}

\def\XiFourb{\tikz[baseline=-1,scale=0.15]{\draw(0,1.5) node[xi] {} -- (0,0); \draw (-1,1) node[xi] {} -- (0,0) node[xi] {} -- (1,1) node[xi] {};}}
\def\XiFourc{\tikz[baseline=2,scale=0.15]{\draw (0,-0.25) node[xi] {} -- (-1,1) node[xi] {} -- (0,2) node[xi] {} -- (-1,3) node[xi] {};}}
\def\XiFoure{\tikz[baseline=0,scale=0.15]{\draw (0,2) node[xi] {} -- (-1,1) node[xi] {} -- (0,0) node[xi] {} -- (1,1) node[xi] {};}}

\colorlet{symbols}{blue!90!black}
\colorlet{testcolor}{green!60!black}
\colorlet{connection}{red!30!black}
\def\symbol#1{\textcolor{symbols}{#1}}
\def\symbol#1{\textcolor{symbols}{#1}}


\tikzset{
root/.style={circle,fill=black!50,inner sep=0pt, minimum size=3mm},
        dot/.style={circle,fill=black,inner sep=0pt, minimum size=1.5mm},
        dotred/.style={circle,fill=black!50,inner sep=0pt, minimum size=2mm},
        var/.style={circle,fill=black!10,draw=black,inner sep=0pt, minimum size=3mm},
        kernel/.style={semithick,shorten >=2pt,shorten <=2pt},
        kernel1/.style={thick},
        kernels/.style={snake=zigzag,shorten >=2pt,shorten <=2pt,segment amplitude=1pt,segment length=4pt,line before snake=2pt,line after snake=5pt,},
		kernels1/.style={snake=zigzag,segment amplitude=0.5pt,segment length=2pt},
		rho1/.style={dotted,semithick},
        rho/.style={densely dashed,semithick,shorten >=2pt,shorten <=2pt},
           testfcn/.style={dotted,semithick,shorten >=2pt,shorten <=2pt},
        renorm/.style={shape=circle,fill=white,inner sep=1pt},
        labl/.style={shape=rectangle,fill=white,inner sep=1pt},
        xic/.style={very thin,circle,fill=symbols,draw=black,inner sep=0pt,minimum size=1.2mm},
        xi/.style={very thin,circle,fill=blue!10,draw=black,inner sep=0pt,minimum size=1.2mm},
        xix/.style={crosscircle,fill=blue!10,draw=black,inner sep=0pt,minimum size=1.2mm},
	xib/.style={very thin,circle,fill=blue!10,draw=black,inner sep=0pt,minimum size=1.6mm},
	xie/.style={very thin,circle,fill=green!50!black,draw=black,inner sep=0pt,minimum size=1mm},
	xid/.style={very thin,circle,fill=symbols,draw=black,inner sep=0pt,minimum size=1.6mm},
	xibx/.style={crosscircle,fill=blue!10,draw=black,inner sep=0pt,minimum size=1.6mm},
	edgetype/.style={very thin,circle,draw=black,inner sep=0pt,minimum size=5mm},
	nodetype/.style={very thick,circle,draw=black,inner sep=0pt,minimum size=5mm},
	kernels2/.style={very thick,draw=connection,segment length=12pt},
clean/.style={thin,circle,fill=black,inner sep=0pt,minimum size=1mm},	not/.style={thin,circle,fill=symbols,draw=connection,fill=connection,inner sep=0pt,minimum size=0.5mm},
	>=stealth,
        }

\tikzset{ individus/.style={scale=0.40,draw,circle,thick,fill=black!10},
 individu/.style={scale=0.40,draw,circle,thick,fill=black!50},       } 
\makeatletter
\def\DeclareSymbol#1#2#3{\expandafter\gdef\csname MH@symb@#1\endcsname{\tikz[baseline=#2,scale=0.15,draw=symbols]{#3}}\expandafter\gdef\csname MH@symb@#1s\endcsname{\scalebox{0.7}{\tikz[baseline=#2,scale=0.15,draw=symbols]{#3}}}}
\def\<#1>{\csname MH@symb@#1\endcsname}
\makeatother

\def\sXi{\symbol{\Xi}} 
 \def\1{\mathbf{\symbol{1}}}
\def\X{\symbol{X}}
 \def\un#1{\hbox{{\indic 1}$_{#1}$}}
\def\one{\mathbf{1}}
\def\eps{\varepsilon}
\def\gep{\varepsilon}

   
\def\MHmakebox#1#2#3{\tikz[baseline=#3,line width=#1,cross/.style={path picture={ 
  \draw[black](path picture bounding box.south) -- (path picture bounding box.north) (path picture bounding box.west) -- (path picture bounding box.east);
}}]{\draw[white] (0,0) rectangle (#2,#2);
\draw[black,cross] (0.1em,0.1em) rectangle (#2-0.1em,#2-0.1em);}}

\def\XI#1{\begin{tikzpicture}[scale=0.2,baseline=0.1cm]
        \node at (0,0)  [dot,color=#1,label=below:] (root) {};
        \node at (0,2)  [dot,color=#1,label=below:] (center) {};
     \draw[rho1,color=#1] (center) to
     node [sloped,below] {\small }     (root);     
     \end{tikzpicture}}

\def\IXi#1{\begin{tikzpicture}[scale=0.2,baseline=0.1cm]
        \node at (0,0)  [dot,color=#1,label=below:] (root) {};
        \node at (0,2)  [dot,color=#1,label=below:] (center) {};
         \draw[kernel1,color=#1] (center) to node [sloped,below] {\small }     (root);
     \end{tikzpicture}}
     
    \def\Xib#1{\begin{tikzpicture}[scale=0.2,baseline=0.1cm]
        \node at (0,0)  [dot,color=#1,label=below:] (root) {};
        \node at (1,2)  [dot,color=#1,label=below:] (right) {};
        \node at (-1,2)  [dot,color=#1,label=below:] (left) {};
         \draw[rho1,color=#1] (right) to
     node [sloped,below] {\small }     (root);
     \draw[rho1,color=#1] (left) to
     node [sloped,below] {\small }     (root);
     \end{tikzpicture}}
     
    \def\XiIXi#1{\begin{tikzpicture}[scale=0.2,baseline=0.1cm]
        \node at (0,0)  [dot,color=#1,label=below:] (root) {};
        \node at (1,2)  [dot,color=#1,label=below:] (right) {};
        \node at (-1,2)  [dot,color=#1,label=below:] (left) {};
         \draw[rho1,color=#1] (right) to
     node [sloped,below] {\small }     (root);
     \draw[kernel1,color=#1] (left) to
     node [sloped,below] {\small }     (root);
     \end{tikzpicture}}

\def\IIXib#1{\begin{tikzpicture}[scale=0.2,baseline=0.1cm]
        \node at (0,0)  [dot,color=#1,label=below:] (root) {};
        \node at (0,2)  [dot,color=#1,label=below:] (rootbis) {};
        \node at (1,4)  [dot,color=#1,label=below:] (right) {};
        \node at (-1,4)  [dot,color=#1,label=below:] (left) {};
         \draw[color=#1,rho1] (right) to
     node [sloped,below] {\small }     (rootbis);
     \draw[color=#1,kernel1] (left) to
     node [sloped,below] {\small }     (rootbis);
     \draw[color=#1,kernel1] (rootbis) to
     node [sloped,below] {\small }     (root);
     \end{tikzpicture}}
     
     \def\IIIXib#1{\begin{tikzpicture}[scale=0.2,baseline=0.1cm]
     \node at (0,0)  [dot,color=#1,label=below:] (root1) {};
        \node at (0,2)  [dot,color=#1,label=below:] (root) {};
        \node at (0,4)  [dot,color=#1,label=below:] (rootbis) {};
        \node at (1,6)  [dot,color=#1,label=below:] (right) {};
        \node at (-1,6)  [dot,color=#1,label=below:] (left) {};
          \draw[color=#1,kernel1] (root) to
     node [sloped,below] {\small }     (root1);
         \draw[color=#1,rho1] (right) to
     node [sloped,below] {\small }     (rootbis);
     \draw[color=#1,kernel1] (left) to
     node [sloped,below] {\small }     (rootbis);
     \draw[color=#1,kernel1] (rootbis) to
     node [sloped,below] {\small }     (root);
     \end{tikzpicture}}
     
     \def\IIXi#1{\begin{tikzpicture}[scale=0.2,baseline=0.1cm]
        \node at (0,0)  [dot,color=#1,label=below:] (root) {};
        \node at (0,2)  [dot,color=#1,label=below:] (rootbis) {};
        \node at (0,4)  [dot,color=#1,label=below:] (center) {};
         \draw[color=#1,kernel1] (center) to
     node [sloped,below] {\small }     (rootbis);
     \draw[color=#1,kernel1] (rootbis) to
     node [sloped,below] {\small }     (root);
     \end{tikzpicture}}
     
     \def\IIIXi#1{\begin{tikzpicture}[scale=0.2,baseline=0.1cm]
        \node at (0,0)  [dot,color=#1,label=below:] (root) {};
        \node at (0,2)  [dot,color=#1,label=below:] (rootbis) {};
        \node at (0,4)  [dot,color=#1,label=below:] (center) {};
        \node at (0,6)  [dot,color=#1,label=below:] (centerbis) {};
         \draw[color=#1,kernel1] (center) to
     node [sloped,below] {\small }     (rootbis);
     \draw[color=#1,kernel1] (centerbis) to
     node [sloped,below] {\small }     (center);
     \draw[color=#1,kernel1] (rootbis) to
     node [sloped,below] {\small }     (root);
     \end{tikzpicture}}
     
     \def\XiIIXi#1{\begin{tikzpicture}[scale=0.2,baseline=0.1cm]
        \node at (0,0)  [dot,color=#1,label=below:] (root) {};
        \node at (-1,2)  [dot,color=#1,label=below:] (left) {};
        \node at (1,2)  [dot,color=#1,label=below:] (right) {};
        \node at (0,4)  [dot,color=#1,label=below:] (leftr) {};
         \draw[color=#1,rho1] (right) to
     node [sloped,below] {\small }     (root);
     \draw[color=#1,kernel1] (left) to
     node [sloped,below] {\small }     (root);
      \draw[color=#1,kernel1] (leftr) to
     node [sloped,below] {\small }     (left);
     \end{tikzpicture}}
     
     \def\IXiIIXi#1{\begin{tikzpicture}[scale=0.2,baseline=0.1cm]
     \node at (0,0)  [dot,color=#1,label=below:] (root1) {};
        \node at (0,2)  [dot,color=#1,label=below:] (root) {};
        \node at (-1,4)  [dot,color=#1,label=below:] (left) {};
        \node at (1,4)  [dot,color=#1,label=below:] (right) {};
        \node at (0,6)  [dot,color=#1,label=below:] (leftr) {};
         \draw[color=#1,rho1] (right) to
     node [sloped,below] {\small }     (root);
     \draw[color=#1,kernel1] (left) to
     node [sloped,below] {\small }     (root);
     \draw[color=#1,kernel1] (root) to
     node [sloped,below] {\small }     (root1);
      \draw[color=#1,kernel1] (leftr) to
     node [sloped,below] {\small }     (left);
     \end{tikzpicture}}
     
     
\def\XiIIXib#1{\begin{tikzpicture}[scale=0.2,baseline=0.1cm]
        \node at (0,0)  [dot,color=#1,label=below:] (root) {};
        \node at (1,2)  [dot,color=#1,label=below:] (right) {};
        \node at (-1,2)  [dot,color=#1,label=below:] (left) {};
        \node at (0,4)  [dot,color=#1,label=below:] (leftr) {};
        \node at (-2,4)  [dot,color=#1,label=below:] (leftl) {};
         \draw[color=#1,rho1] (right) to
     node [sloped,below] {\small }     (root);
     \draw[color=#1,kernel1] (left) to
     node [sloped,below] {\small }     (root);
     \draw[color=#1,rho1] (leftr) to
     node [sloped,below] {\small }     (left);
     \draw[color=#1,kernel1] (leftl) to
     node [sloped,below] {\small }     (left);
     \end{tikzpicture}}
     
     \def\IXiIIXib#1{\begin{tikzpicture}[scale=0.2,baseline=0.1cm]
     \node at (0,0)  [dot,color=#1,label=below:] (rootbis) {};
        \node at (0,2)  [dot,color=#1,label=below:] (root) {};
        \node at (1,4)  [dot,color=#1,label=below:] (right) {};
        \node at (-1,4)  [dot,color=#1,label=below:] (left) {};
        \node at (0,6)  [dot,color=#1,label=below:] (leftr) {};
        \node at (-2,6)  [dot,color=#1,label=below:] (leftl) {};
         \draw[color=#1,kernel1] (root) to
     node [sloped,below] {\small }     (rootbis);
         \draw[color=#1,rho1] (right) to
     node [sloped,below] {\small }     (root);
     \draw[color=#1,kernel1] (left) to
     node [sloped,below] {\small }     (root);
     \draw[color=#1,rho1] (leftr) to
     node [sloped,below] {\small }     (left);
     \draw[color=#1,kernel1] (leftl) to
     node [sloped,below] {\small }     (left);
     \end{tikzpicture}}
     \def\XiIXiIIXibc#1{\begin{tikzpicture}[scale=0.2,baseline=0.1cm]
     
     \node at (2,2)  [dot,color=#1,label={[label distance=-0.2em]above: \scriptsize  $ \ell_4 $}] (rightbis) {};
     \node at (1,0)  [dot,color=#1,label=below:] (rootbis) {};
        \node at (0,2)  [dot,color=#1,label=below:] (root) {};
        \node at (1,4)  [dot,color=#1,label={[label distance=-0.2em]above: \scriptsize  $ \ell_3 $} ] (right) {};
        \node at (-1,4)  [dot,color=#1,label=below:] (left) {};
        \node at (0,6)  [dot,color=#1,label={[label distance=-0.2em]above: \scriptsize  $ \ell_2 $}] (leftr) {};
        \node at (-2,6)  [dot,color=#1,label={[label distance=-0.2em]above: \scriptsize  $ \ell_1 $}] (leftl) {};
         \draw[color=#1,kernel1] (root) to
     node [sloped,below] {\small }     (rootbis);
         \draw[color=#1,rho1] (right) to
     node [sloped,below] {\small }     (root);
     \draw[color=#1,rho1] (rightbis) to
     node [sloped,below] {\small }     (rootbis);
     \draw[color=#1,kernel1] (left) to
     node [sloped,below] {\small }     (root);
     \draw[color=#1,rho1] (leftr) to
     node [sloped,below] {\small }     (left);
     \draw[color=#1,kernel1] (leftl) to
     node [sloped,below] {\small }     (left);
     \end{tikzpicture}}
     
     \def\XiIXiIIXib#1{\begin{tikzpicture}[scale=0.2,baseline=0.1cm]
     
     \node at (2,2)  [dot,color=#1,label=below:] (rightbis) {};
     \node at (1,0)  [dot,color=#1,label=below:] (rootbis) {};
        \node at (0,2)  [dot,color=#1,label=below:] (root) {};
        \node at (1,4)  [dot,color=#1,label=below:] (right) {};
        \node at (-1,4)  [dot,color=#1,label=below:] (left) {};
        \node at (0,6)  [dot,color=#1,label=below:] (leftr) {};
        \node at (-2,6)  [dot,color=#1,label=below:] (leftl) {};
         \draw[color=#1,kernel1] (root) to
     node [sloped,below] {\small }     (rootbis);
         \draw[color=#1,rho1] (right) to
     node [sloped,below] {\small }     (root);
     \draw[color=#1,rho1] (rightbis) to
     node [sloped,below] {\small }     (rootbis);
     \draw[color=#1,kernel1] (left) to
     node [sloped,below] {\small }     (root);
     \draw[color=#1,rho1] (leftr) to
     node [sloped,below] {\small }     (left);
     \draw[color=#1,kernel1] (leftl) to
     node [sloped,below] {\small }     (left);
     \end{tikzpicture}}
     
     \def\IXib#1{\begin{tikzpicture}[scale=0.2,baseline=0.1cm]
        \node at (0,0)  [dot,color=#1,label=below:$  $] (root) {};
         \node at (2,2)  [dot,color=#1,label=right:] (right) {};
         \node at (-2,2)  [dot,color=#1,label=left: ] (left) {};
         \node at (-3,4)  [dot,color=#1,label={[label distance=-0.2em]above: \scriptsize  $ \ell_1 $}] (leftl) {};
          \node at (-1,4)  [dot,color=#1,label={[label distance=-0.2em]above: \scriptsize  $ \ell_2 $} ] (leftr) {};
          \node at (1,4)  [dot,color=#1,label={[label distance=-0.2em]above: \scriptsize  $ \ell_3 $}  ] (rightl) {};
           \node at (3,4)  [dot,color=#1,label={[label distance=-0.2em]above: \scriptsize  $ \ell_4 $} ] (rightr) {};
            \draw[color=#1,kernels1] (right) to
     node [sloped,below] {\small }     (root); \draw[color=#1,kernels1] (left) to
     node [sloped,below] {\small }     (root);
     \draw[rho1,color=#1] (leftr) to
     node [sloped,below] {\small }     (left);
      \draw[kernel1,color=#1] (rightr) to
     node [sloped,below] {\small }     (right);
      \draw[rho1,color=#1] (rightl) to
     node [sloped,below] {\small }     (right);
      \draw[kernel1,color=#1] (leftl) to
     node [sloped,below] {\small }     (left);
     \end{tikzpicture}}
    
\DeclareMathOperator*{\bplus}{
\tikzexternaldisable
\mathchoice{\MHmakebox{.17ex}{1.5em}{0.48em}}{\MHmakebox{.12ex}{1.1em}{0.28em}}{}{}
\tikzexternalenable
}


%TCIDATA{OutputFilter=LATEX.DLL}
%TCIDATA{Version=5.50.0.2953}
%TCIDATA{<META NAME="SaveForMode" CONTENT="1">}
%TCIDATA{BibliographyScheme=Manual}
%TCIDATA{Created=Wednesday, March 09, 2016 07:57:09}
%TCIDATA{LastRevised=Wednesday, March 09, 2016 09:12:56}
%TCIDATA{<META NAME="GraphicsSave" CONTENT="32">}
%TCIDATA{<META NAME="DocumentShell" CONTENT="Standard LaTeX\Blank - Standard LaTeX Article">}
%TCIDATA{CSTFile=40 LaTeX article.cst}

\newtheorem{theorem}{Theorem}
\newtheorem{acknowledgement}[theorem]{Acknowledgement}
\newtheorem{algorithm}[theorem]{Algorithm}
\newtheorem{axiom}[theorem]{Axiom}
\newtheorem{case}[theorem]{Case}
\newtheorem{claim}[theorem]{Claim}
\newtheorem{conclusion}[theorem]{Conclusion}
\newtheorem{condition}[theorem]{Condition}
\newtheorem{conjecture}[theorem]{Conjecture}
\newtheorem{corollary}[theorem]{Corollary}
\newtheorem{criterion}[theorem]{Criterion}
\newtheorem{definition}[theorem]{Definition}
\newtheorem{example}[theorem]{Example}
\newtheorem{exercise}[theorem]{Exercise}
\newtheorem{lemma}[theorem]{Lemma}
\newtheorem{notation}[theorem]{Notation}
\newtheorem{problem}[theorem]{Problem}
\newtheorem{proposition}[theorem]{Proposition}
%\newenvironment{proof}[1][Proof]{\noindent\textbf{#1.} }{\ \rule{0.5em}{0.5em}}

\theoremstyle{remark}
\newtheorem{remark}[theorem]{Remark}
\newtheorem{solution}[theorem]{Solution}
\newtheorem{summary}[theorem]{Summary}



\newcommand{\Nr}{\textnormal{Nr}}
\newcommand{\Vol}{\textnormal{Vol}}
\newcommand{\Tr}{\textnormal{Tr}}
\newcommand{\Cl}{\textnormal{Cl}}
\newcommand{\Hom}{\textnormal{Hom}}
\newcommand{\End}{\textnormal{End}}
\newcommand{\Ker}{\textnormal{Ker}}
\newcommand{\Aut}{\textnormal{Aut}}
\newcommand{\Sh}{\textnormal{Shuffle}}
\newcommand{\Id}{\textnormal{Id}}
\newcommand{\diam}{\textnormal{diam}}
\newcommand{\Diag}{\textnormal{Diag}}
\newcommand{\ExpSig}{\textnormal{ESig}}
\newcommand{\supp}{\textnormal{supp}}
\newcommand{\Lip}{\textnormal{Lip}}
\newcommand{\sign}{\textnormal{sign}}
\newcommand{\loc}{\textnormal{loc}}
\newcommand{\Lie}{\textnormal{Lie}}
\newcommand{\Vect}{\textnormal{Vect}}
\newcommand{\diver}{\textnormal{div}}
\newcommand{\stat}{\textnormal{stat}}
\newcommand{\op}{\textnormal{op}}
\newcommand{\Real}{\textnormal{Re}}

\newcommand{\GPrimal}{T(\R^{1+d})}
\newcommand{\GDual}{T((\R^{1+d}))}
\newcommand{\BPrimal}{\HH}
\newcommand{\BDual}{\HH^*}
\newcommand{\extract}{\delta}

\newcommand{\Deltam}{\Delta^{\!-}}
\newcommand{\Deltap}{\Delta^{\!+}}
\newcommand{\Deltashuff}{\Delta_{\shuffle}}
\newcommand{\tensor}{{\dot\otimes}}
\newcommand{\poly}{\odot}


\newcommand{\OO}{\mathcal{O}}
\newcommand{\QQ}{\mathcal{Q}}
\newcommand{\RR}{\mathcal{R}}
\newcommand{\II}{\mathcal{I}}
\newcommand{\TT}{\mathcal{T}}
\newcommand{\CC}{\mathcal{C}}
\newcommand{\PP}{\mathcal{P}}
\newcommand{\DD}{\mathcal{D}}
\newcommand{\EE}{\mathcal{E}}
\newcommand{\HH}{\mathcal{H}}
\newcommand{\FF}{\mathcal{F}}
\newcommand{\GG}{\mathcal{G}}
\newcommand{\BB}{\mathcal{B}}
\newcommand{\LL}{\mathcal{L}}
\newcommand{\VV}{\mathcal{V}}
\newcommand{\UU}{\mathcal{U}}
\newcommand{\MM}{\mathcal{M}}
\newcommand{\NN}{\mathcal{N}}
\newcommand{\KK}{\mathcal{K}}
\newcommand{\SSS}{\mathcal{S}}
\newcommand{\A}{\mathcal{A}}
\newcommand{\WW}{\mathcal{W}}

\newcommand{\R}{\mathbb R}
\newcommand{\C}{\mathbb C}
\newcommand{\N}{\mathbb N}
\newcommand{\Z}{\mathbb Z}
\newcommand{\Q}{\mathbb Q}
\newcommand{\F}{\mathbb F}
\newcommand{\K}{\mathbb K}
\newcommand{\T}{\mathbb T}
\newcommand{\W}{\mathbb W}
\newcommand{\Pbb}{\mathbb P}
\newcommand{\Xbb}{\mathbb X}
\newcommand{\Abb}{\mathbb A}
\newcommand{\Ybb}{\mathbb Y}

\newcommand{\Xbf}{\mathbf X}
\newcommand{\Y}{\mathbf Y}
\newcommand{\x}{\mathbf x}
\newcommand{\y}{\mathbf y}
\newcommand{\z}{\mathbf z}
\newcommand{\w}{\mathbf w}
\newcommand{\mm}{\mathbf m}
\newcommand{\hh}{\mathbf h}
\newcommand{\B}{\mathbf B}
\newcommand{\ZZ}{\mathbf Z}
\newcommand{\WWW}{\mathbf W}
\newcommand{\bpi}{\mathbf \Pi}

\newcommand{\G}{G}

\newcommand{\var}[1]{#1\textnormal{-var}}
\newcommand{\Hol}[1]{#1\textnormal{-H{\"o}l}}
\newcommand{\pvar}{p\textnormal{-var}}
\newcommand{\pprimevar}{p'\textnormal{-var}}
\newcommand{\qvar}{q\textnormal{-var}}
\newcommand{\onevar}{1\textnormal{-var}}
\newcommand{\twovar}{2\textnormal{-var}}
\newcommand{\rhovar}{\rho\textnormal{-var}}
\newcommand{\aHol}{\alpha\textnormal{-H{\"o}l}}
\newcommand{\pHol}{1/p\textnormal{-H{\"o}l}}
\newcommand{\pprimeHol}{1/p'\textnormal{-H{\"o}l}}
\newcommand{\qHol}{1/q\textnormal{-H{\"o}l}}
\newcommand{\betaHol}{\beta\textnormal{-H{\"o}l}}
\newcommand{\aprimeHol}{\alpha'\textnormal{-H{\"o}l}}
\newcommand{\oneHol}{1\textnormal{-H{\"o}l}}

\newcommand{\EEE}[1]{\mathbb E \left[ #1 \right]}
\newcommand{\EEEover}[2]{\mathbb E^{#1} \left[ #2 \right]}
\newcommand{\PPPover}[2]{\mathbb P^{#1} \left[ #2 \right]}
\newcommand{\EEEunder}[2]{\mathbb E_{#1} \left[ #2 \right]}
\newcommand{\Var}[1]{\textnormal{Var} \left[ #1 \right]}
\newcommand{\Diff}{\textnormal{Diff}}
\newcommand{\Homeo}{\textnormal{Homeo}}
\newcommand{\PPP}[1]{\mathbb{P} \left[ #1 \right]}
\newcommand{\QQQ}[1]{\Q \left[ #1 \right]}
\newcommand{\cv}[1]{\textnormal{cv}\left( #1 \right)}
\newcommand{\ob}[1]{\textnormal{ob}\left( #1 \right)}
\newcommand{\spn}[1]{\textnormal{span}\left( #1 \right)}
\newcommand{\id}{\textnormal{id}}
\newcommand{\norm}[1]{\left|\left|#1 \right|\right|}
\newcommand{\normt}[1]{\left|\left|\left|#1 \right|\right|\right|}
\newcommand{\norms}[1]{\left|#1 \right|}
\newcommand{\normc}{\norm{\cdot}}
\newcommand{\normtc}{\normt{\cdot}}
%\newcommand{\1}[1]{\mathbf 1 \{#1\}}
\newcommand{\0}{\mathbf 0}
\newcommand{\LLL}{\mathbf L}
\newcommand{\GL}{\mathbf{GL}}
\newcommand{\LMC}{\mathbf{LMC}}
\newcommand{\Lyons}{S}

\newcommand{\uu}{\mathfrak u}
\newcommand{\g}{\mathfrak g}
\newcommand{\llie}{\mathfrak l}
\newcommand{\h}{\mathfrak h}
\newcommand{\gl}{\mathfrak {gl}}
\newcommand{\su}{\mathfrak{su}}
\newcommand{\symp}{\mathfrak{sp}}
\newcommand{\m}{\mathfrak m}

\newcommand{\gen}[1]{\langle #1 \rangle}
\newcommand{\floor}[1]{\lfloor #1 \rfloor}
\newcommand{\roof}[1]{\lceil #1 \rceil}

\newcommand{\midset}{\,\middle|\,}

\newcommand\restr[2]{{\left.\kern-\nulldelimiterspace % automatically resize the bar with \right
  #1 % the function
  \vphantom{\big|} % pretend it's a little taller at normal size
  \right|_{#2} % this is the delimiter
  }}

\def\eqd{\,{\buildrel \DD \over =}\,}
\def\neqd{\,{\buildrel \DD \over \neq}\,}
\def\convd{\,{\buildrel \DD \over \rightarrow}\,}
